Nonparametric augmented probability weighting with sparsity

Nonresponse frequently arises in practice, and simply ignoring it may lead to erroneous inference. Besides, the number of collected covariates may increase as the sample size in modern statistics, so parametric imputation or propensity score weighting usually leads to inefficiency without consideration of sparsity. In this paper, we propose a nonparametric imputation method with sparse learning by employing an efficient kernel-based learning gradient algorithm to identify truly informative covariates. Moreover, an augmented probability weighting framework is adopted to improve the estimation efficiency of the nonparametric imputation method and establish the limiting distribution of the corresponding estimator under regularity assumptions. The performance of the proposed method is also supported by several simulated examples and one real-life analysis.

==> notations.tex <==
%=================================================
%-------------------------------- my symbols ------------------------------------
%=================================================

%-------------------- brackets ---------------------

\newcommand{\Norm}[1]{\left\Vert #1\right\Vert}			%	operator norm
\newcommand{\Inner}[2]{\left\langle #1, #2 \right\rangle}	%	inner product
\newcommand{\Abs}[1]{\left\vert#1\right\vert}			%	absolute value
\newcommand{\vect}[1]{\boldsymbol{#1}}				%	vector
%\newcommand{\matr}[1]{\mathcal{#1}}				%	matrix


%---------------- math operators -----------------

\newcommand{\tp}{{\rm T}}						%	transpose
\newcommand{\sgn}{{\rm sgn}}						%	sign
\newcommand{\tr}{{\rm tr}}						%	trace
\newcommand{\cov}{{\rm Cov}}						%	covariance
\newcommand{\diag}{{\rm diag}}					%	diagonal
\newcommand{\var}{{\rm Var}}						%	variance
\newcommand{\med}{{\rm med}}					%	median
\newcommand{\card}{{\rm Card}}					%	cardinality
\newcommand{\diff}{\mathrm{d}}					%	differential
\newcommand{\argmin}[1]{\mathop{\rm{argmin}}_{#1}}	%	argmin
\newcommand{\argmax}[1]{\mathop{\rm{argmax}}_{#1}}	%	argmax
											
\newcommand*\widebar[1]{\,						%	widebar
	\hbox{%
   		\kern0.01em%
		\vbox{%
			\hrule height 0.5pt		%	The actual bar
			\kern0.33ex			%	Distance between bar and symbol
			\hbox{%
				\kern-0.1em		%	Shortening on the left side
				\ensuremath{#1}%
				\kern-0.1em		%	Shortening on the right side
			}%
		}%
	}%
\,}%
\let\hat\widehat
\let\tilde\widetilde
\let\bar\widebar

\newcommand{\etal}{\mbox{\sl et al.\;}}
\newcommand{\ie}{\mbox{\sl i.e.\;}}					
\newcommand{\eg}{\mbox{\sl e.g.\;}}					%	example


%=================================================
%------------------------ Proper noun abbreviation ---------------------------
%=================================================

\newcommand{\AR}{{\rm AR}}
\newcommand{\MA}{{\rm MA}}
\newcommand{\ARMA}{{\rm ARMA}}
\newcommand{\AAR}{{\rm AAR}}
\newcommand{\ARIMA}{{\rm ARIMA}}
\newcommand{\FAR}{{\rm FAR}}
\newcommand{\ARCH}{{\rm ARCH}}
\newcommand{\GARCH}{{\rm GARCH}}
\newcommand{\Beta}{{\rm Beta}}
\newcommand{\DLS}{{\mbox{\scriptsize DLS}}}
\newcommand{\IRSC}{{\rm IRSC}}
\newcommand{\IID}{{\rm IID}}
\newcommand{\Leb}{{\rm Leb}}
\newcommand{\LK}{{\mbox{\scriptsize LK}}}
\newcommand{\LKopt}{{\mbox{\scriptsize LK, OPT}}}
\newcommand{\LS}{{\mbox{\scriptsize LS}}}
\newcommand{\LSopt}{{\mbox{\scriptsize LS, OPT}}}
\newcommand{\MISE}{{\rm MISE}}
\newcommand{\MSE}{{\rm MSE}}
\newcommand{\STD}{{\rm STD}}
\newcommand{\MSPE}{{\rm MSPE}}
\newcommand{\MAE}{{\rm MAE}}
\newcommand{\MAD}{{\rm MAD}}
\newcommand{\RSS}{{\rm RSS}}
\newcommand{\WN}{{\rm WN}}
\newcommand{\abias}{{\rm AB}}
\newcommand{\avar}{{\rm AV}}
\newcommand{\vech}{{\rm vech}}
\newcommand{\bias}{{\rm Bias}}
\newcommand{\sopt}{\mbox{{\scriptsize opt}}}
\newcommand{\AIC}{{\rm AIC}}
\newcommand{\BIC}{{\rm BIC}}
\newcommand{\BICP}{{\rm BICP}}
\newcommand{\BICC}{{\rm BICC}}



%=================================================
%----------------------------------- boldface --------------------------------------
%=================================================

%---------------- bold capital letters -----------------

\newcommand{\bA}{{\mathbf A}}
\newcommand{\bB}{{\mathbf B}}
\newcommand{\bC}{{\mathbf C}}
\newcommand{\bD}{{\mathbf D}}
\newcommand{\bE}{{\mathbf E}}
\newcommand{\bF}{{\mathbf F}}
\newcommand{\bG}{{\mathbf G}}
\newcommand{\bH}{{\mathbf H}}
\newcommand{\bI}{{\mathbf I}}
\newcommand{\bJ}{{\mathbf J}}
\newcommand{\bK}{{\mathbf K}}
\newcommand{\bL}{{\mathbf L}}
\newcommand{\bM}{{\mathbf M}}
\newcommand{\bN}{{\mathbf N}}
\newcommand{\bO}{{\mathbf O}}
\newcommand{\bP}{{\mathbf P}}
\newcommand{\bQ}{{\mathbf Q}}
\newcommand{\bR}{{\mathbf R}}
\newcommand{\bS}{{\mathbf S}}
\newcommand{\bT}{{\mathbf T}}
\newcommand{\bU}{{\mathbf U}}
\newcommand{\bV}{{\mathbf V}}
\newcommand{\bW}{{\mathbf W}}
\newcommand{\bX}{{\mathbf X}}
\newcommand{\bY}{{\mathbf Y}}
\newcommand{\bZ}{{\mathbf Z}}


%---------------- bold lower case letters -----------------

\newcommand{\ba}{{\mathbf a}}
\newcommand{\bb}{{\mathbf b}}
\newcommand{\bd}{{\mathbf d}}
\newcommand{\bc}{{\mathbf c}}
\newcommand{\be}{{\mathbf e}}
\newcommand{\bff}{{\mathbf f}}
\newcommand{\bg}{{\mathbf g}}
\newcommand{\bh}{{\mathbf h}}
\newcommand{\bi}{{\mathbf i}}
\newcommand{\bj}{{\mathbf j}}
\newcommand{\bk}{{\mathbf k}}
\newcommand{\bll}{{\mathbf l}}
\newcommand{\bmm}{{\mathbf m}}
\newcommand{\bnn}{{\mathbf n}}
\newcommand{\boo}{{\mathbf o}}
\newcommand{\bpp}{{\mathbf p}}
\newcommand{\bq}{{\mathbf q}}
\newcommand{\br}{{\mathbf r}}
\newcommand{\bs}{{\mathbf s}}
\newcommand{\bt}{{\mathbf t}}
\newcommand{\bu}{{\mathbf u}}
\newcommand{\bv}{{\mathbf v}}
\newcommand{\bw}{{\mathbf w}}
\newcommand{\bx}{{\mathbf x}}
\newcommand{\by}{{\mathbf y}}
\newcommand{\bz}{{\mathbf z}}


%---------------- bold Greek letters -----------------

\newcommand{\balpha} {\boldsymbol{\alpha}}

\newcommand{\bbeta}  {\boldsymbol{\beta}}
\newcommand{\bBeta}  {\boldsymbol{\Beta}}
\newcommand{\bfeta}  {\boldsymbol{\eta}}

\newcommand{\bvarphi}  {\boldsymbol{\varphi}}

\newcommand{\bdelta} {\boldsymbol{\delta}}
\newcommand{\bDelta}{\boldsymbol{\Delta}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\bLambda} {\boldsymbol{\Lambda}}
\newcommand{\bepsilon}{\bolsymbol{\epsilon}}

\newcommand{\bomega}{\boldsymbol{\omega}}
\newcommand{\bOmega}{\boldsymbol{\Omega}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\bSigma}{\boldsymbol{\Sigma}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}
\newcommand{\bGamma} {\boldsymbol{\Gamma}}
\newcommand{\brho}{\mbox{\boldmath$\rho$}}
\newcommand{\bRho} {\boldsymbol{\Rho}}
\newcommand{\btheta} {\boldsymbol{\theta}}
\newcommand{\bTheta} {\boldsymbol{\Theta}}

\newcommand{\bPhi} {\boldsymbol{\Phi}}

\newcommand{\bPsi} {\boldsymbol{\Psi}}

\newcommand{\bxi} {\boldsymbol{\xi}}
\newcommand{\bpsi} {\boldsymbol{\psi}}
\newcommand{\bmu} {\boldsymbol{\mu}}
\newcommand{\bzeta} {\boldsymbol{\zeta}}
\newcommand{\bnu}{\boldsymbol{\nu}}
%\newcommand{\bve}{\mbox{\boldmath$\varepsilon$}}


\newcommand{\bzero}{{\mathbf 0}}


%=================================================
%----------------------------------- mathcal{} -------------------------------------
%=================================================
											%
\newcommand{\mcA}{{\mathcal A}}
\newcommand{\mcB}{{\mathcal B}}					%	Byzantine machine
\newcommand{\mcC}{{\mathcal C}}
\newcommand{\mcD}{{\mathcal D}}
\newcommand{\mcE}{{\mathcal E}}
\newcommand{\mcF}{{\mathcal F}}
\newcommand{\mcG}{{\mathcal G}}
\newcommand{\mcH}{{\mathcal H}}					%	saperate machines
\newcommand{\mcI}{{\mathcal I}}
\newcommand{\mcJ}{{\mathcal J}}
\newcommand{\mcK}{{\mathcal K}}
\newcommand{\mcL}{{\mathcal L}}					%	loss function
\newcommand{\mcM}{{\mathcal M}}
\newcommand{\mcN}{{\mathcal N}}					%	standard normal distribution
\newcommand{\mcO}{{\mathcal O}}
\newcommand{\mcP}{{\mathcal P}}
\newcommand{\mcQ}{{\mathcal Q}}
\newcommand{\mcR}{{\mathcal R}}
\newcommand{\mcS}{{\mathcal S}}
\newcommand{\mcT}{{\mathcal T}}
\newcommand{\mcU}{{\mathcal U}}
\newcommand{\mcV}{{\mathcal V}}
\newcommand{\mcW}{{\mathcal W}}
\newcommand{\mcX}{{\mathcal X}}
\newcommand{\mcY}{{\mathcal Y}}
\newcommand{\mcZ}{{\mathcal Z}}


%=================================================
%----------------------------------- mathbb{} -------------------------------------
%=================================================

\newcommand{\mbA}{{\mathbb A}}
\newcommand{\mbB}{{\mathbb B}}					%	ball
\newcommand{\mbC}{{\mathbb C}}					%	complex field
\newcommand{\mbD}{{\mathbb D}}
\newcommand{\mbE}{{\mathbb E}}					%	expectation
\newcommand{\mbF}{{\mathbb F}}
\newcommand{\mbG}{{\mathbb G}}
\newcommand{\mbH}{{\mathbb H}}
\newcommand{\mbI}{{\mathbb I}}					%	indicator function
\newcommand{\mbJ}{{\mathbb J}}
\newcommand{\mbK}{{\mathbb K}}
\newcommand{\mbL}{{\mathbb L}}
\newcommand{\mbM}{{\mathbb M}}
\newcommand{\mbN}{{\mathbb N}}
\newcommand{\mbO}{{\mathbb O}}
\newcommand{\mbP}{{\mathbb P}}					%	probability
\newcommand{\mbQ}{{\mathbb Q}}					%	rational field
\newcommand{\mbR}{{\mathbb R}}					%	real field
\newcommand{\mbS}{{\mathbb S}}					%	sphere
\newcommand{\mbT}{{\mathbb T}}
\newcommand{\mbU}{{\mathbb U}}
\newcommand{\mbV}{{\mathbb V}}
\newcommand{\mbW}{{\mathbb W}}
\newcommand{\mbX}{{\mathbb X}}
\newcommand{\mbY}{{\mathbb Y}}
\newcommand{\mbZ}{{\mathbb Z}}					%	integer ring


%=================================================
%----------------------------------- mathfrak{} ------------------------------------
%=================================================

\newcommand{\mfA}{{\mathfrak A}}
\newcommand{\mfB}{{\mathfrak B}}
\newcommand{\mfC}{{\mathfrak C}}
\newcommand{\mfD}{{\mathfrak D}}
\newcommand{\mfE}{{\mathfrak E}}					%	cai-liu exponential
\newcommand{\mfF}{{\mathfrak F}}
\newcommand{\mfG}{{\mathfrak G}}
\newcommand{\mfH}{{\mathfrak H}}
\newcommand{\mfI}{{\mathfrak I}}
\newcommand{\mfJ}{{\mathfrak J}}
\newcommand{\mfK}{{\mathfrak K}}
\newcommand{\mfL}{{\mathfrak L}}
\newcommand{\mfM}{{\mathfrak M}}
\newcommand{\mfN}{{\mathfrak N}}					%	epsilon Nets
\newcommand{\mfO}{{\mathfrak O}}
\newcommand{\mfP}{{\mathfrak P}}
\newcommand{\mfQ}{{\mathfrak Q}}
\newcommand{\mfR}{{\mathfrak R}}
\newcommand{\mfS}{{\mathfrak S}}
\newcommand{\mfT}{{\mathfrak T}}
\newcommand{\mfU}{{\mathfrak U}}
\newcommand{\mfV}{{\mathfrak V}}
\newcommand{\mfW}{{\mathfrak W}}
\newcommand{\mfX}{{\mathfrak X}}					%	set of samples
\newcommand{\mfY}{{\mathfrak Y}}
\newcommand{\mfZ}{{\mathfrak Z}}


%=================================================
%---------------- Euler math fonts/ package: euscript ---------------------
%=================================================



\newcommand{\eulA}{\EuScript A}
\newcommand{\eulB}{\EuScript B}
\newcommand{\eulC}{\EuScript C}
\newcommand{\eulD}{\EuScript D}
\newcommand{\eulE}{\EuScript E}
\newcommand{\eulF}{\EuScript F}
\newcommand{\eulG}{\EuScript G}
\newcommand{\eulH}{\EuScript H}
\newcommand{\eulI}{\EuScript I}
\newcommand{\eulJ}{\EuScript J}
\newcommand{\eulK}{\EuScript K}
\newcommand{\eulL}{\EuScript L}
\newcommand{\eulM}{\EuScript M}
\newcommand{\eulN}{\EuScript N}
\newcommand{\eulO}{\EuScript O}
\newcommand{\eulP}{\EuScript P}
\newcommand{\eulQ}{\EuScript Q}
\newcommand{\eulR}{\EuScript R}
\newcommand{\eulS}{\EuScript S}
\newcommand{\eulT}{\EuScript T}
\newcommand{\eulU}{\EuScript U}
\newcommand{\eulV}{\EuScript V}
\newcommand{\eulW}{\EuScript W}
\newcommand{\eulX}{\EuScript X}
\newcommand{\eulY}{\EuScript Y}
\newcommand{\eulZ}{\EuScript Z}

\DeclareMathAlphabet\EuScriptBF{U}{eus}{b}{n}

\newcommand{\eulbA}{\EuScriptBF A}
\newcommand{\eulbB}{\EuScriptBF B}
\newcommand{\eulbC}{\EuScriptBF C}
\newcommand{\eulbD}{\EuScriptBF D}
\newcommand{\eulbE}{\EuScriptBF E}
\newcommand{\eulbF}{\EuScriptBF F}
\newcommand{\eulbG}{\EuScriptBF G}
\newcommand{\eulbH}{\EuScriptBF H}
\newcommand{\eulbI}{\EuScriptBF I}
\newcommand{\eulbJ}{\EuScriptBF J}
\newcommand{\eulbK}{\EuScriptBF K}
\newcommand{\eulbL}{\EuScriptBF L}
\newcommand{\eulbM}{\EuScriptBF M}
\newcommand{\eulbN}{\EuScriptBF N}
\newcommand{\eulbO}{\EuScriptBF O}
\newcommand{\eulbP}{\EuScriptBF P}
\newcommand{\eulbQ}{\EuScriptBF Q}
\newcommand{\eulbR}{\EuScriptBF R}
\newcommand{\eulbS}{\EuScriptBF S}
\newcommand{\eulbT}{\EuScriptBF T}
\newcommand{\eulbU}{\EuScriptBF U}
\newcommand{\eulbV}{\EuScriptBF V}
\newcommand{\eulbW}{\EuScriptBF W}
\newcommand{\eulbX}{\EuScriptBF X}
\newcommand{\eulbY}{\EuScriptBF Y}
\newcommand{\eulbZ}{\EuScriptBF Z}


%=================================================
%--------------- Math script fonts/ package: mathrsfs ---------------------
%=================================================

\newcommand{\mathA}{\mathscr A}
\newcommand{\mathB}{\mathscr B}
\newcommand{\mathC}{\mathscr C}
\newcommand{\mathD}{\mathscr D}
\newcommand{\mathE}{\mathscr E}
\newcommand{\mathF}{\mathscr F}
\newcommand{\mathG}{\mathscr G}
\newcommand{\mathH}{\mathscr H}
\newcommand{\mathI}{\mathscr I}
\newcommand{\mathJ}{\mathscr J}
\newcommand{\mathK}{\mathscr K}
\newcommand{\mathL}{\mathscr L}
\newcommand{\mathM}{\mathscr M}
\newcommand{\mathN}{\mathscr N}
\newcommand{\mathO}{\mathscr O}
\newcommand{\mathP}{\mathscr P}
\newcommand{\mathQ}{\mathscr Q}
\newcommand{\mathR}{\mathscr R}
\newcommand{\mathS}{\mathscr S}
\newcommand{\mathT}{\mathscr T}
\newcommand{\mathU}{\mathscr U}
\newcommand{\mathV}{\mathscr V}
\newcommand{\mathW}{\mathscr W}
\newcommand{\mathX}{\mathscr X}
\newcommand{\mathY}{\mathscr Y}
\newcommand{\mathZ}{\mathscr Z}

